News Without Borders: Domain Adaptation of Multilingual Sentence Embeddings for Cross-lingual News Recommendation

Rapidly growing numbers of multilingual news consumers pose an increasing challenge to news recommender systems in terms of providing customized recommendations. First, existing neural news recommenders, even when powered by multilingual language models (LMs), suffer substantial performance losses in zero-shot cross-lingual transfer (ZS-XLT). Second, the current paradigm of fine-tuning the backbone LM of a neural recommender on task-specific data is computationally expensive and infeasible in few-shot recommendation and cold-start setups, where data is scarce or completely unavailable. In this work, we propose a news-adapted sentence encoder (NaSE), domain-specialized from a pretrained massively multilingual sentence encoder (SE). To this end, we construct and leverage PolyNews and PolyNewsParallel, two multilingual news-specific corpora. With the news-adapted multilingual SE in place, we test the effectiveness of (i.e., question the need for) supervised fine-tuning for news recommendation, and propose a simple and strong baseline based on (i) frozen NaSE embeddings and (ii) late click-behavior fusion. We show that NaSE achieves state-of-the-art performance in ZS-XLT in true cold-start and few-shot news recommendation.

==> tables/fsxlt_rec.tex <==
\begin{table*}
    \centering

    \caption{\zsxlt{} performance in few-shot recommendation (i.e., for different number of impressions used in training). For each model, we report performance (i) on the English MIND dataset (denoted \texttt{ENG}), (ii) averaged across all 14 target languages in \xmind{} (denoted \texttt{AVG}), and (iii) the relative percentage difference between average \zsxlt{} and \texttt{ENG} performance ($\%\Delta$). We report averages and standard deviations across three runs.}
    \label{tab:fs_xlt_rec}
    
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lcgacgacgacga}
        \toprule
        \multirow{2}{*}{\textbf{Model}}
        & \multicolumn{3}{c}{\textbf{AUC}} & \multicolumn{3}{c}{\textbf{MRR}} 
        & \multicolumn{3}{c}{\textbf{nDCG@5}} & \multicolumn{3}{c}{\textbf{nDCG@10}} 
        \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}

        & ENG & AVG & $\%\Delta$ 
        & ENG & AVG & $\%\Delta$ 
        & ENG & AVG & $\%\Delta$ 
        & ENG & AVG & $\%\Delta$ \\ \hline

        \multicolumn{13}{l}{\textit{\textbf{10-shots}}} \\
        
        \lfrecscl\textsubscript{\labse}
        & 51.02$\pm$0.06 % AUC ENG
        & 51.17$\pm$0.02 % AUC AVG
        & +0.30 %Delta
        & 31.17$\pm$0.16  % MRR ENG
        & 29.02$\pm$0.08  % MRR AVG
        & -6.90 % Delta
        & 28.88$\pm$0.18  % nDCG@5 ENG
        & 26.70$\pm$0.11% nDCG@5 AVG
        & -7.57 % Delta
        & 35.11$\pm$0.18  % nDCG@10 ENG
        & 33.01$\pm$0.10  % nDCG@10 AVG
        & -5.96 % Delta
        \\

        \lfrecscl\textsubscript{\nase}
        & 61.62$\pm$0.58 % AUC ENG
        & 61.40$\pm$0.50 % AUC AVG
        & -0.35 % Delta
        & 33.54$\pm$0.30  % MRR ENG
        & 32.98$\pm$0.26  % MRR AVG
        & -1.69 % Delta
        & 31.66$\pm$0.33  % nDCG@5 ENG
        & 31.02$\pm$0.27 % nDCG@5 AVG
        & -2.03 % Delta
        & 37.70$\pm$0.28  % nDCG@10 ENG
        & 37.15$\pm$0.25  % nDCG@10 AVG
        & -1.44 % Delta
        \\

        \naml\textsubscript{\labse}
        & 56.19$\pm$0.41 % AUC ENG
        & 55.13$\pm$0.95 % AUC AVG
        & -1.89 % Delta
        & 33.14$\pm$0.18  % MRR ENG
        & 31.56$\pm$0.96  % MRR AVG
        & -4.75 % Delta
        & 31.18$\pm$0.14  % nDCG@5 ENG
        & 29.34$\pm$1.02 % nDCG@5 AVG
        & -5.89 % Delta
        & 37.23$\pm$0.18  % nDCG@10 ENG
        & 35.63$\pm$1.01  % nDCG@10 AVG
        & -4.31 % Delta
        \\

        \naml\textsubscript{\nase}
        & 54.50$\pm$0.52 % AUC ENG
        & 54.51$\pm$0.37 % AUC AVG
        & +0.01 % Delta
        &  33.21$\pm$0.37 % MRR ENG
        & 32.76$\pm$0.35  % MRR AVG
        & -1.34 % Delta
        & 31.26$\pm$0.56  % nDCG@5 ENG
        & 30.94$\pm$0.43% nDCG@5 AVG
        & -1.01% Delta
        & 37.31$\pm$0.55  % nDCG@10 ENG
        & 37.04$\pm$0.41  % nDCG@10 AVG
        & -0.70 % Delta
        \\ \hline

        \multicolumn{13}{l}{\textit{\textbf{50-shots}}} \\
        
        \lfrecscl\textsubscript{\labse}
        & 61.07$\pm$1.19 % AUC ENG
        & 59.04$\pm$0.59 % AUC AVG
        & -3.32 % Delta
        & 32.36$\pm$0.51  % MRR ENG
        & 30.94$\pm$0.29  % MRR AVG
        & -4.37 % Delta
        & 30.52$\pm$0.62  % nDCG@5 ENG
        & 29.03$\pm$0.33 % nDCG@5 AVG
        & -4.90 % Delta
        & 36.69$\pm$0.63  % nDCG@10 ENG
        & 35.26$\pm$0.30  % nDCG@10 AVG
        & -3.87 % Delta
        \\

        \lfrecscl\textsubscript{\nase}
        & 61.55$\pm$1.05 % AUC ENG
        & 59.24$\pm$0.89 % AUC AVG
        & -3.75 % Delta
        & 33.17$\pm$0.39  % MRR ENG
        & 31.77$\pm$0.39  % MRR AVG
        & -4.22 % Delta
        & 31.37$\pm$0.49  % nDCG@5 ENG
        & 29.84$\pm$0.41% nDCG@5 AVG
        & -4.87 % Delta
        & 37.43$\pm$0.47  % nDCG@10 ENG
        & 35.98$\pm$0.40  % nDCG@10 AVG
        & -3.88 % Delta
        \\

        \naml\textsubscript{\labse}
        & 55.50$\pm$1.13 % AUC ENG
        & 54.57$\pm$0.67 % AUC AVG
        & -1.67 % Delta
        & 32.93$\pm$0.85  % MRR ENG
        & 31.54$\pm$0.56 % MRR AVG
        & -4.23 % Delta
        & 31.15$\pm$0.91  % nDCG@5 ENG
        & 29.26$\pm$0.55 % nDCG@5 AVG
        & -5.75 % Delta
        & 37.21$\pm$0.87  % nDCG@10 ENG
        & 35.60$\pm$0.52  % nDCG@10 AVG
        & -4.32 % Delta
        \\

        \naml\textsubscript{\nase}
        & 53.32$\pm$0.21 % AUC ENG
        & 53.47$\pm$0.38 % AUC AVG
        & +0.28 % Delta
        & 33.31$\pm$0.39  % MRR ENG
        & 33.10$\pm$0.42  % MRR AVG
        & -0.64 % Delta
        & 31.42$\pm$0.32  % nDCG@5 ENG
        & 31.24$\pm$0.36 % nDCG@5 AVG
        & -0.59 % Delta
        & 37.49$\pm$0.32  % nDCG@10 ENG
        & 37.33$\pm$0.38  % nDCG@10 AVG
        & -0.41 % Delta
        \\ \hline

        \multicolumn{13}{l}{\textit{\textbf{100-shots}}} \\
        
        \lfrecscl\textsubscript{\labse}
        & 61.20$\pm$0.72 % AUC ENG
        & 59.54$\pm$0.43 % AUC AVG
        & -2.72% Delta
        & 33.19$\pm$0.72  % MRR ENG
        & 31.10$\pm$0.58 % MRR AVG
        & -6.27 % Delta
        & 31.25$\pm$0.80  % nDCG@5 ENG
        & 29.07$\pm$0.60 % nDCG@5 AVG
        & -6.97 % Delta
        & 37.34$\pm$0.73  % nDCG@10 ENG
        & 35.32$\pm$0.53  % nDCG@10 AVG
        & -5.42 % Delta
        \\

        \lfrecscl\textsubscript{\nase}
        & 62.29$\pm$1.03 % AUC ENG
        & 59.85$\pm$0.72 % AUC AVG
        & -3.92% Delta
        & 33.40$\pm$0.42  % MRR ENG
        & 32.07$\pm$0.42  % MRR AVG
        & -3.97 % Delta
        & 31.36$\pm$0.60  % nDCG@5 ENG
        & 29.99$\pm$0.45 % nDCG@5 AVG
        & -4.36 % Delta
        & 37.52$\pm$0.64  % nDCG@10 ENG
        &  36.17$\pm$0.45 % nDCG@10 AVG
        & -3.61 % Delta
        \\

        \naml\textsubscript{\labse}
        & 55.67$\pm$0.94 % AUC ENG
        & 54.15$\pm$0.81 % AUC AVG
        & -2.72 % Delta
        & 34.24$\pm$0.52  % MRR ENG
        & 31.41$\pm$0.86  % MRR AVG
        & -8.26 % Delta
        & 32.45$\pm$0.61  % nDCG@5 ENG
        & 29.18$\pm$0.90 % nDCG@5 AVG
        & -10.06% Delta
        & 38.33$\pm$0.61  % nDCG@10 ENG
        & 35.40$\pm$0.88  % nDCG@10 AVG
        & -7.65 % Delta
        \\

        \naml\textsubscript{\nase}
        & 52.98$\pm$0.34 % AUC ENG
        & 53.38$\pm$0.39 % AUC AVG
        & +0.75 % Delta
        & 33.92$\pm$0.20  % MRR ENG
        & 34.04$\pm$0.22  % MRR AVG
        & +0.37 % Delta
        & 31.90$\pm$0.18  % nDCG@5 ENG
        & 32.06$\pm$0.22 % nDCG@5 AVG
        & +0.50 % Delta
        & 37.96$\pm$0.23  % nDCG@10 ENG
        & 38.05$\pm$0.27  % nDCG@10 AVG
        & +0.23 % Delta
        \\

        
    \bottomrule
    \end{tabular}%
    }
    
    \vspace{-1em}
\end{table*}


==> tables/zsxlt_rec_ablate_finetuning.tex <==
\begin{table*}
    \centering

    \caption{\zsxlt{} recommendation performance with full vs. partial fine-tuning of the backbone \xlmrbase. For each model, we report performance (i) on the English MIND dataset (\texttt{ENG}), and (ii) averaged across all 14 target languages in \xmind{} (\texttt{AVG}). We report averages, standard deviations across three runs.}
    \label{tab:zs_xlt_rec_ablate_finetuning}

    
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lcgcgcgcg}
        \toprule
        \multirow{2}{*}{\textbf{Model}}
        & \multicolumn{2}{c}{\textbf{AUC}} & \multicolumn{2}{c}{\textbf{MRR}} 
        & \multicolumn{2}{c}{\textbf{nDCG@5}} & \multicolumn{2}{c}{\textbf{nDCG@10}} 
        \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}

        & ENG & AVG 
        & ENG & AVG 
        & ENG & AVG 
        & ENG & AVG  \\ \hline

        NAML\textsubscript{CAT}
        & \multicolumn{2}{c}{55.46$\pm$0.18}  % AUC 
        & \multicolumn{2}{c}{31.12$\pm$0.56}  % MRR 
        & \multicolumn{2}{c}{29.44$\pm$0.67}  % nDCG@5 
        & \multicolumn{2}{c}{35.81$\pm$0.59}  % nDCG@10 
        \\ \hdashline
        
       
        NAML\textsubscript{\xlmr\textsubscript{12layers}}
        & 50.00$\pm$0.02 % AUC ENG
        &  49.99$\pm$0.02% AUC AVG
        &  30.33$\pm$0.94 % MRR ENG
        &  29.87$\pm$0.79% MRR AVG
        &  28.41$\pm$0.98 % nDCG@5 ENG
        & 27.96$\pm$0.97% nDCG@5 AVG
        &  34.72$\pm$0.75 % nDCG@10 ENG
        &  34.34$\pm$0.84 % nDCG@10 AVG
        \\

        NAML\textsubscript{\xlmr\textsubscript{4layers}}
        & 52.85$\pm$2.27  % AUC ENG
        & 52.49$\pm$2.60 % AUC AVG
        & 35.98$\pm$0.44  % MRR ENG
        & 33.98$\pm$0.95  % MRR AVG
        & 34.11$\pm$0.46 % nDCG@5 ENG
        & 32.13$\pm$1.08 % nDCG@5 AVG
        & 40.43$\pm$0.39  % nDCG@10 ENG
        & 38.38$\pm$1.02  % nDCG@10 AVG
        \\

        \hdashline

        MINS\textsubscript{\xlmr\textsubscript{12layers}}
        & 50.81$\pm$1.18 % AUC ENG
        &  50.87$\pm$1.10% AUC AVG
        &  29.03$\pm$2.78 % MRR ENG
        &  29.26$\pm$2.69 % MRR AVG
        &  27.10$\pm$2.85 % nDCG@5 ENG
        & 27.36$\pm$2.74% nDCG@5 AVG
        &  33.60$\pm$2.79 % nDCG@10 ENG
        &  33.72$\pm$2.64 % nDCG@10 AVG
        \\

        MINS\textsubscript{\xlmr\textsubscript{4layers}}
        & 59.89$\pm$0.29  % AUC ENG
        & 56.94$\pm$1.40 % AUC AVG
        & 34.75$\pm$0.24  % MRR ENG
        & 33.11$\pm$0.51  % MRR AVG
        & 32.94$\pm$0.23  % nDCG@5 ENG
        & 31.32$\pm$0.52 % nDCG@5 AVG
        & 39.35$\pm$0.20  % nDCG@10 ENG
        & 37.64$\pm$0.50  % nDCG@10 AVG
        \\

        \hdashline

        CAUM\textsubscript{\xlmr\textsubscript{12layers}}
        & 54.14$\pm$0.71 % AUC ENG
        &  54.18$\pm$1.06% AUC AVG
        & 29.91$\pm$0.53  % MRR ENG
        &  29.94$\pm$044 % MRR AVG
        &  27.93$\pm$0.56 % nDCG@5 ENG
        & 27.90$\pm$0.49% nDCG@5 AVG
        & 34.47$\pm$0.53  % nDCG@10 ENG
        & 34.50$\pm$0.46  % nDCG@10 AVG
        \\

        CAUM\textsubscript{\xlmr\textsubscript{4layers}}
        & 57.82$\pm$3.01  % AUC ENG
        & 55.90$\pm$1.75 % AUC AVG
        & 32.92$\pm$1.68  % MRR ENG
        & 31.38$\pm$1.62  % MRR AVG
        & 31.09$\pm$1.88  % nDCG@5 ENG
        & 29.60$\pm$1.76 % nDCG@5 AVG
        & 37.49$\pm$1.71  % nDCG@10 ENG
        & 35.96$\pm$1.58  % nDCG@10 AVG
        \\

        \hdashline

        MaNNER\textsubscript{\xlmr\textsubscript{12layers}}
        & 50.00$\pm$0.00 % AUC ENG
        & 50.00$\pm$0.00 % AUC AVG
        & 31.34$\pm$1.92  % MRR ENG
        & 29.80$\pm$2.38  % MRR AVG
        & 29.39$\pm$1.75  % nDCG@5 ENG
        & 27.87$\pm$2.25% nDCG@5 AVG
        & 35.78$\pm$1.94  % nDCG@10 ENG
        & 34.17$\pm$2.18  % nDCG@10 AVG
        \\

        MaNNER\textsubscript{\xlmr\textsubscript{4layers}}
        & 50.00$\pm$0.00  % AUC ENG
        & 50.00$\pm$0.00 % AUC AVG
        & 35.58$\pm$0.31  % MRR ENG
        & 33.03$\pm$0.54  % MRR AVG
        & 33.86$\pm$0.22  % nDCG@5 ENG
        & 31.34$\pm$0.48 % nDCG@5 AVG
        & 40.17$\pm$0.21  % nDCG@10 ENG
        & 37.64$\pm$0.44  % nDCG@10 AVG
        \\

    \bottomrule
    \end{tabular}
    }
    
    \vspace{-0.5em}
\end{table*}

